MERMAID: Metaphor Generation with Symbolism and Discriminative Decoding

Generating metaphors is a challenging task as it requires a proper understanding of abstract concepts, making connections between unrelated concepts, and deviating from the literal meaning. In this paper, we aim to generate a metaphoric sentence given a literal expression by replacing relevant verbs. Based on a theoretically-grounded connection between metaphors and symbols, we propose a method to automatically construct a parallel corpus by transforming a large number of metaphorical sentences from the Gutenberg Poetry corpus (Jacobs, 2018) to their literal counterpart using recent advances in masked language modeling coupled with commonsense inference. For the generation task, we incorporate a metaphor discriminator to guide the decoding of a sequence to sequence model fine-tuned on our parallel data to generate high-quality metaphors. Human evaluation on an independent test set of literal statements shows that our best model generates metaphors better than three well-crafted baselines 66% of the time on average. A task-based evaluation shows that human-written poems enhanced with metaphors proposed by our model are preferred 68% of the time compared to poems without metaphors.

==> approach.tex <==
\section{MERMAID: Metaphor Generation with Symbolism and Discriminative Decoding }
% \smnote{Since use of COMET is in parallel data creation, I would argue that your entire approach is MERMAID (so that should be the title of this section instead of approach. Then I would remove section title "Data" and just have two subsection 1) "Parallel Data Creation" (and here you have the use of COMET) and 2) Metaphor Generation with Discriminative Decoding.  You can introduce Test Data in Evaluation section.}
Our approach for metaphor generation from literal descriptive sentences has three steps: 1) first convert potential metaphorical sentences from a large scale poetry corpus into literal sentences using Masked Language Models and structured common sense symbolism (Section \ref{section:data}); 2) given the \textit{[literal sentence, metaphorical sentence]} pairs, fine-tune a seq2seq model on these pairs to generate a metaphorical sentence given a literal sentence (Section \ref{section:model}). This two-step approach is shown in the upper half of Figure \ref{figure:sim}.
